Bayesian Persuasion Meets Mechanism Design: Going Beyond Intractability with Type Reporting

Bayesian persuasion studies how an informed sender should partially disclose information so as to influence the behavior of self-interested receivers. In the last years, a growing attention has been devoted to relaxing the assumption that the sender perfectly knows receiver's payoffs. The first crucial step towards such an achievement is to study settings where each receiver's payoffs depend on their unknown type, which is randomly determined by a known finite-supported probability distribution. This begets considerable computational challenges, as computing a sender-optimal signaling scheme is inapproximable up to within any constant factor. In this work, we circumvent this issue by leveraging ideas from mechanism design. In particular, we introduce a type reporting step in which the receiver is asked to report their type to the sender, after the latter has committed to a menu defining a signaling scheme for each possible receiver's type. We prove that, with a single receiver, the addition of this type reporting stage makes the sender's computational problem tractable. Then, we extend our framework to settings with multiple receivers, focusing on the case of no inter-agent externalities and binary actions. We show that it is possible to find a sender-optimal solution in polynomial-time by means of the ellipsoid method, given access to a suitable polynomial-time separation oracle. This can be implemented for supermodular and anonymous sender's utility functions. As for the case of submodular sender's utility functions, we first approximately cast the sender's problem into a linearly-constrained mathematical program whose objective function is the multi-linear extension of the sender's utility. Then, we show how to find in polynomial-time an approximate solution to the program by means of a continuous greedy algorithm. This provides a (1 -1/e)-approximation to the problem.

==> independent.tex <==
\section{Independent Types}

We can solve a slightly different problem.

\begin{subequations} \label{lp:multiInd}
	\begin{align}
	max_{\phi\ge0,x\ge0} \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec} \phi_\theta(R) f_\theta(R) \\
	\sum_{R \subseteq \rec:r \in R} \phi_\theta(R)  = \sum_{k_r} \lambda_{k_r} x^{r,k_r}_\theta \forall \kvec \in \bar \K, \theta,r \in \rec \label{lp:multi1Ind}\\
	\sum_{\theta \in \Theta} \mu_\theta x^{r,k}_\theta u^k_\theta(a_1) +\sum_\theta \in \Theta \mu_\theta (1-x^{r,k}_\theta) u^k_\theta(a_0) \ge l^{r,k,k'}_{a_1}+l^{r,k,k'}_{a_0} \forall r \in \rec, k\neq k' \in \K_r \label{lp:multi2Ind}\\
	l^{r,k,k'}_{a_1} \ge \sum_{\theta \in \Theta} \mu_\theta x^{r,k'}_\theta u^k_\theta(a) \forall r \in \rec,a \in \A_r,k,k' \in \K_r \label{lp:multi3Ind}\\
	l^{r,k,k'}_{a_0} \ge \sum_{\theta \in \Theta} \mu_\theta (1-x^{r,k'}_\theta) u^k_\theta(a) \forall r \in \rec,a \in \A_r,k,k' \in \K_r \label{lp:multi4ind}\\
	\sum_{\theta \in \Theta} \mu_\theta x^{r,k}_\theta [u^k_\theta(a_1) -u^k_\theta(a_0)] \ge 0 \forall r \in \rec,k \in \K_r \label{lp:multi5Ind}\\
	\sum_\theta \mu_{\theta \in \Theta} (1-x^{r,k}_\theta) [u^k_\theta(a_0) -u^k_\theta(a_1)] \ge 0 \forall r \in \rec,k \in \K_r \label{lp:multi6Ind}\\
	\sum_{R \subseteq \rec}  \phi_\theta(R) = 1 \forall \theta \in \Theta \label{lp:multi7Ind} 
	\end{align}
\end{subequations}

\begin{lemma}
	The value of LP \ref{lp:multiInd} is at least the value of the optimal signaling scheme.
\end{lemma}

\begin{proof}
	By Theorem \ref{thm:direct}, the optimal signaling scheme is given by the solution of LP \ref{lp:multi} in which $\lambda_\kvec=\prod_{r}\lambda_{k_r}$.
	We show that $\phi_\theta(R)=\sum_\kvec \lambda_\kvec \phi^\kvec_\theta(R)$ is a feasible solution, concluding the proof.
	For each $r$
	\[\sum_{R \subseteq \rec:r \in R} \phi_\theta(R) =\sum_{R \subseteq \rec:r \in R}\sum_\kvec \lambda_\kvec \phi^\kvec_\theta(R)=\sum_\kvec \lambda_\kvec \sum_{R \subseteq \rec:r \in R} \phi^\kvec_\theta(R)= \sum_\kvec \lambda_\kvec x^{r,k_r}_\theta= \sum_{k_r} \lambda_{k_r} x^{r,k_r}_\theta  \]
\end{proof}

Finally, we show how to build a menu of signaling scheme by a solution to LP \ref{lp:multiInd}.

\begin{lemma}
	Given a solution to LP \ref{lp:multiInd}, we can recover in polynomial time a menu of signaling scheme with the same value.
\end{lemma}

\begin{proof}
	Given a vector of reported type, we choose the signaling scheme $\phi^\kvec_\theta(R)$ that solves the following LP.
	
	\begin{subequations} \label{lp:multiIndT}
		\begin{align}
		max_{\phi^\kvec\ge0} \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec} \phi^{\kvec}_\theta(R) f_\theta(R) \\
		\sum_{R \subseteq \rec:r \in R} \phi^\kvec_\theta(R)  =  x^{r,k_r}_\theta \forall \theta,r \in \rec \label{lp:multi1IndT}\\
		\sum_{R \subseteq \rec}  \phi_\theta^\kvec(R) = 1 \forall \theta \in \Theta \label{lp:multi7IndT} 
		\end{align}
	\end{subequations}
Hence, the algorithm has utility at least 
	\begin{subequations} \label{lp:multiIndT}
	\begin{align}
	max_{\phi^\kvec\ge0} \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec} f_\theta(R) \sum_{\kvec} \lambda_\kvec \phi^{\kvec}_\theta(R)  \\
	\sum_{R \subseteq \rec:r \in R} \phi^\kvec_\theta(R)  =  x^{r,k_r}_\theta \forall \theta,r \in \rec \label{lp:multi1IndT}\\
	\sum_{R \subseteq \rec}  \phi_\theta^\kvec(R) = 1 \forall \theta \in \Theta \label{lp:multi7IndT} 
	\end{align}
\end{subequations}

The solution is feasible to

	\begin{subequations} \label{lp:multiIndT}
	\begin{align}
	max_{\phi^\kvec\ge0} \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec} f_\theta(R) \sum_{\kvec} \lambda_\kvec \phi^{\kvec}_\theta(R)  \\
	\sum_{\kvec} \lambda_\kvec \sum_{R \subseteq \rec:r \in R} \phi^\kvec_\theta(R)  =  \sum_{\kvec} \lambda_\kvec  x^{r,k_r}_\theta \forall \theta,r \in \rec \label{lp:multi1IndT}\\
	\sum_{R \subseteq \rec}  \phi_\theta^\kvec(R) = 1 \forall \theta \in \Theta \label{lp:multi7IndT} 
	\end{align}
\end{subequations}

Replacing $\sum_{\kvec} \lambda_\kvec \sum_{R \subseteq \rec:r \in R} \phi^\kvec_\theta(R) =\phi_\theta(R)$ we obtain a solution to LP initial.




	
	%\begin{comment}
	$\phi_\theta(R) =\prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{k_r} \lambda_{k_r}x^{r,\kvec}_\theta)}$. \footnote{The signaling scheme cannot be computed before the type reporting step. Indeed, there are an exponential number of possible type profiles.}
	The expected utility is given by \[\sum_{\kvec} \lambda_\kvec \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec} \phi^{\kvec}_\theta(R) f_\theta(R)= \sum_{\kvec} \lambda_\kvec  \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec}  f_\theta(R) \phi_\theta(R) \prod_{r\in \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{k_r} x^{r,\kvec}_\theta}=\sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec}  f_\theta(R) \phi_\theta(R) \sum_{\kvec} \lambda_\kvec\prod_{r\in \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{k_r} x^{r,\kvec}_\theta} \]
	\[=\sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec}  f_\theta(R) \phi_\theta(R) \sum_{\kvec} \lambda_\kvec \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} x^{r,\kvec}_\theta} \prod_{r\in \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{k_r} x^{r,\kvec}_\theta}= \sum_{\theta \in \Theta} \mu_\theta \sum_{R \subseteq \rec}  f_\theta(R) \phi_\theta(R)\]
	Moreover, the signaling schemes are consistent since 
	\[\sum_{R \subseteq \rec}  \phi_\theta^\kvec(R)=\sum_{R \subseteq \rec} \phi_\theta(R) \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)}\]
	\[= \sum_{R \subseteq \rec} \phi_\theta(R) \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{ \sum_{R \in \rec:r \in R} \phi_\theta(R)} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{R \in \rec:r \in R} \phi_\theta(R)} = \]
		\[= \sum_{R \subseteq \rec\setminus\{i\}} \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{ \sum_{R \in \rec:r \in R} \phi_\theta(R)} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{1-\sum_{R \in \rec:r \in R} \phi_\theta(R)} [\phi_\theta(R\cup \{i\})  \frac{ x^{i,\kvec}_\theta}{ \sum_{R \in \rec:i \in R} \phi_\theta(R)} +\phi_\theta(R)\frac{ 1-x^{i,\kvec}_\theta}{1-\sum_{R \in \rec:i \in R} \phi_\theta(R)} ]= \]
	%\end{comment}
	
	
	By induction on the number of receivers.
	Let \[\gamma^{i,\kvec}_\theta= \sum_{R \subseteq \rec^i} \phi^i_\theta(R) \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)}\].
	%we show that $\gamma^{i,\kvec}_\theta=1$.
	
	With receiver $i=1$.
	$\gamma^{i,\kvec}_\theta= \phi^1_\theta(1)  \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} + \phi^1_\theta(\emptyset)  \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)}=1$
	
	With $i>1$
	\[\gamma^{i,\kvec}_\theta=\sum_{R \subseteq \rec^{i-1}}[\phi_\theta^{i}(R\cup \{i\})  \frac{ x^{i,\kvec}_\theta}{ \sum_{R \in \rec:i \in R} \phi_\theta(R)}\prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)}+ \]
	\[+\sum_{R \subseteq \rec^{i-1}}[\phi_\theta^{i}(R)  \frac{ x^{i,\kvec}_\theta}{ \sum_{R \in \rec:i \in R} \phi_\theta(R)}\prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)}\]
	
	
	\[   \sum_{R \subseteq \rec^{i-1}} \prod_{r\in R} \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r} x^{r,\kvec}_\theta} \prod_{r \notin R} \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)} [\phi_\theta^{i}(R\cup \{i\}) \frac{ x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(x^{r,\kvec}_\theta)} + \phi_\theta^{i}(R) \frac{ 1-x^{r,\kvec}_\theta}{\sum_{k_r} \lambda_{k_r}(1-x^{r,\kvec}_\theta)} ] + \]
	
\end{proof}



==> online.tex <==
\section{Multi Receiver Online}

Action space is huge and number of types is exponential in the instance size.
So, we reduce the problem to a learning problem in a small decision space.
The main idea is that the sender must commit only to the marginal signaling scheme before observing the receivers'types.
The computation of the signaling scheme is an optimization problem when the marginal signaling schemes and the receivers' types are known.
So we can work on the smaller decision space of the marginal signaling schemes. 

In particular, the action space of the learner is a given $P\subset \mathbb{R}^{\nType N}$ and the utility is a given function $g^{\kvec}:X\rightarrow [0,1]$  depending only on the vector $x \in P$.
%, while the utility function is given by $g^{\kvec}:X\rightarrow [0,1]$.
%$P$ is the polytope of $x$ defined by the following inequalities.
%\begin{align}
%x^\theta_{i,k}=\sum_{\pvec:a^{i,k}(\pvec)=a_1} \gamma^{i,k}_{\pvec} \pvec_\theta / \mu_\theta\\
%\sum_{\pvec} \gamma^{i,k}_{\pvec} \pvec u^{i,k}(a^{i,k}(\pvec)) \ge \sum_{\pvec} \gamma^{i,k'}_{\pvec} \pvec u^{i,k}(a^{i,k}(\pvec))  \forall k\neq k' \in \Theta \\
%\sum_{\pvec} \gamma^{i,k}_{\pvec} \pvec_\theta =\mu_\theta \forall  \theta \in \Theta,i, k\\
%\gamma\ge 0
%\end{align}

%\begin{align}
%\sum_a \sum_\theta \mu_\theta x_{r,k,\theta} u^k_\theta(a) \ge \sum_a l^k_{a} \\
%l^k_{a}\ge \sum_\theta \mu_\theta x_{r,k,\theta} u^k_\theta(a') \forall a'\\
%\sum_\theta \mu_\theta x_{r,k,\theta} [u^k_\theta(a) -u^k_\theta(a')] \ge 0\\
%\sum_\theta x_{r,k,\theta}=1
%\end{align}


The function $g^\kvec(x)=\sum_\theta \mu_\theta l(x^{\theta,\kvec})$ and $l(x)=max_{y \in \Delta_s} f(s)$ s.t. $\sum_{S:i\in S} y_s=x$, where $x^{\theta,\kvec}$ is the vector with $x_i=x^{i,k_i}_\theta$.
Notice that $l(x)$ is exactly the concave closure of f and it is concave.

our general approach works as follow.

\begin{algorithm}[H]\caption{\textsc{no-regret Algorithm}}
	\begin{algorithmic}[1]
		\State$\Phi^1=$any signaling scheme
		\For{ $t=1$ to $T$}
		\State Play $\Phi^t$
		\State observes the receivers types $\kvec^t$
		\State $\phi$  optimal signaling scheme with marginal $\{\Phi^{r,k^t_r}\}_{r \in R}$
		\State $\Phi^{t+1}$ learning($\kvec^t$)
		\EndFor
	\end{algorithmic}	\label{alg:computePrices}
\end{algorithm}

\begin{theorem}
	Given a no-regret algorithm, there exists a no-regret algorithm.
\end{theorem}

\begin{proof}
	Let $\Phi^*$ be the optimal marginal signaling schemes.
	By the property of the no-regret algorithm, $\sum_t [u(\phi^\kvec) - u(\phi^t)]=\sum_t [max u(\phi^\kvec) - max u(\phi^t) = \sum_t g(\phi)-g(\phi)\le $ regret first algorithm.
\end{proof}
%It is easy to see that the two problems are equivalent.
%Formally, we show that
%(1)Given a signaling scheme $\Phi$, there exists a vector x such that $  u^\kvec(\phi^\kvec,\kvec)\le f^\kvec(x)$ for each $\kvec$.
%
%(2)given a vector $x$ there exists a signaling scheme $\Phi$ with $  u^\kvec(\phi^\kvec,\kvec) = \sum_\kvec \lambda_\kvec f^\kvec(x)$. Moreover the signaling scheme $\Phi$ is direct.
%
%\begin{lemma}
%	(1)
%\end{lemma}
%
%\begin{proof}
%	Let $\Phi$ be a signaling scheme.
%	Let $x^{\theta}_{i,k}=\sum_{s:\pvec^s\in \pvec^{i,k,a_1}} \phi_\theta(s)$.
%	Let $\gamma^i,k,\pvec$
%	Given a vector $\kvec$, let $y^\theta_S=\sum_{s:\pvec^s\in \pvec^{i,k,a_1} \forall s \in S} \phi_\theta(s)$.
%	Then, the utility of the signaling scheme is $\sum_\theta \sum_S y^{\theta}(s) u^s(S)\le concave\ closure $ since ...
%\end{proof}
%
%\begin{lemma}
%	(2)
%\end{lemma}
%
%\begin{proof}
%	We show how to build a signaling scheme $\Phi$ given a vector x.
%	$\phi^\kvec_\theta(S)= y^{\theta}_{S}$.
%	$\phi^{k_r}_\theta(a_1)=x^{\theta}_{r,k}$.
%\end{proof}




\section{a learning algorithm for problem x with supermodular and anonymous functions}

We choose to adopt a general frameworks that works with every possible function, so we do not take advantage from the concavity  of the function.
As an alternative, we can use similar ideas to design a gradient descent procedure.

To employ the result of \cite{suggalaOnline2020}, we need an oracle that solve the following problem.
\begin{align}
max_{x \in P} \sum_t  f^{k^t} (x) + \sum_{\theta,i,k}\sigma_{\theta,i,k} x^{\theta}_{i,k}
\end{align}
This is exactly the LP of previous section and can be computed in polynomial time.
Moreover, Given the marginal signaling scheme we can compute the optimal signaling scheme with a smaller problem in which we fixed the marginal signaling schemes.

As a last step we need to prove that $f^\kvec$ is Lisptick continuous.

\begin{lemma}
	for each possible function $f^\kvec$, $x$,$y$, $|f^\kvec(x)-f^\kvec(y)|\le ||x-y||_1$.
\end{lemma}

\begin{proof}
	VERAMENTE?
\end{proof}


\subsection{a polynomial time no-$(1-1/e)^2$-regret for submodular functions}

work on the multilinear extension of LP ...

$$max \sum_\theta \mu_\theta F_\theta(x^{\kvec,\theta})$$
$$x \in P$$

It is well known that the correlation gap is at most $1-1/e$ and hence the optimal solution that signals indipendently is at least $1-1/e$.
The problem is online maximization of a continuos DR-submodular function.
There is a no-$1-1/e$-regret on the multi-linear extension.

\textcolor{red}{COME AVERE UNA 1-1/e APPROXIMATION?????????????????????????}


